The Power of Nondeterminism in Self-Assembly

We investigate the role of nondeterminism in Winfree's abstract Tile Assembly Model (aTAM), which was conceived to model artificial molecular self-assembling systems constructed from DNA. Of particular practical importance is to find tile systems that minimize resources such as the number of distinct tile types, each of which corresponds to a set of DNA strands that must be custom-synthesized in actual molecular implementations of the aTAM. We seek to identify to what extent the use of nondeterminism in tile systems affects the resources required by such molecular shape-building algorithms. We first show a "molecular computability theoretic" result: there is an infinite shape S that is uniquely assembled by a tile system but not by any deterministic tile system. We then show an analogous phenomenon in the finitary "molecular complexity theoretic" case: there is a finite shape S that is uniquely assembled by a tile system with c tile types, but every deterministic tile system that uniquely assembles S has more than c tile types. In fact we extend the technique to derive a stronger (classical complexity theoretic) result, showing that the problem of finding the minimum number of tile types that uniquely assemble a given finite shape is Sigma-P-2-complete. In contrast, the problem of finding the minimum number of deterministic tile types that uniquely assemble a shape was shown to be NP-complete by Adleman, Cheng, Goel, Huang, Kempe, Moisset de Espan\'es, and Rothemund (Combinatorial Optimization Problems in Self-Assembly, STOC 2002). The conclusion is that nondeterminism confers extra power to assemble a shape from a small tile system, but unless the polynomial hierarchy collapses, it is computationally more difficult to exploit this power by finding the size of the smallest tile system, compared to finding the size of the smallest deterministic tile system.

==> intro.tex <==
\section{Introduction}
\label{sec-intro}

Tile self-assembly is an algorithmically rich model of ``programmable crystal growth''.
It is possible to design molecules (square-like ``tiles'') with specific binding sites so that, even subject to the chaotic nature of molecules floating randomly in a well-mixed chemical soup, they are guaranteed to bind so as to deterministically form a single target shape.
This is despite the number of different types of tiles possibly being much smaller than the size of the shape and therefore having only ``local information'' to guide their attachment.
The ability to control nanoscale structures and machines to atomic-level precision will rely crucially on sophisticated self-assembling systems that automatically control their own behavior where no top-down externally controlled device could fit.

A practical implementation of self-assembling molecular tiles was proved experimentally feasible in 1982 by Seeman \cite{Seem82} using DNA complexes formed from artificially synthesized strands.
%, originally as an attempt to facilitate the crystallization step of x-ray diffraction crystallography.
Experimental advances have delivered increasingly reliable assembly of algorithmic DNA tiles with error rates of 10\% per tile in 2004 \cite{RoPaWi04}, 1.4\% per tile in 2007 \cite{FujHarParWinMur07}, and 0.13\% per tile in 2009 \cite{BarSchRotWin09}.
Erik Winfree \cite{Winf98} introduced the abstract Tile Assembly Model (aTAM) -- based on a constructive version of Wang tiling \cite{Wang61,Wang63} -- as a simplified mathematical model of self-assembling DNA tiles.
Winfree demonstrated the computational universality of the aTAM by showing how to simulate an arbitrary cellular automaton with a tile assembly system.
Building on these connections to computability, Rothemund and Winfree \cite{RotWin00} investigated a self-assembly resource bound known as \emph{tile complexity}, the minimum number of tile types needed to assemble a shape.
They showed that for most $n$, the problem of assembling an $n \times n$ square has tile complexity $\Omega\left(\frac{\log n}{\log \log n}\right)$, and Adleman, Cheng, Goel, and Huang \cite{AdChGoHu01} exhibited a construction showing that this lower bound is asymptotically tight.
%\opt{normal}{Under natural generalizations of the model such as those studied by Aggarwal, Cheng, Goldwasser, Kao, Moisset de Espan\'{e}s, and Schweller \cite{AGKS05}, as well as Becker, Rapaport, and R{\'e}mila \cite{BeckerRR06}, Kao and Schweller \cite{KaoSchS08,KS06}, Demaine, Demaine, Fekete, Ishaque, Rafalin, Schweller, and Souvaine \cite{DDFIRSS07}, Summers \cite{Sum09}, Doty \cite{RSAES}, Chandran, Gopalkrishnan, and Reif \cite{ChaGopRei09}, Abel, Benbernou, Damian, Demaine, Demaine, Flatland, Kominers, and Schweller \cite{RNaseSODA2010}, and Demaine, Patitz, Schweller, and Summers \cite{DemPatSchSum2010RNase}, tile complexity can be reduced for tasks such as square-building and assembly of more general shapes.}
Under natural generalizations of the model \cite{AGKS05, BeckerRR06, KaoSchS08, KS06, DDFIRSS07, Sum09, RSAES, ChaGopRei09, RNaseSODA2010, DemPatSchSum2010RNase, SolWin07, ManStaSto09ISAAC}, tile complexity can be reduced for tasks such as square-building and assembly of more general shapes.
%Experimental success in the self-assembly of DNA tiles has increased steadily over the past decade
%\cite{RoPaWi04, BarSchRotWin09, CheSchGoeWin07, MaoLabReiSee00, WinLiuWenSee98, LiuShaSee99, MaoSunSee99, LiuParReiLab04, YanFenLabRei03, FujHarParWinMur07}.
%Coupled with physical
%\cite{ChenEtAl04n, MLR07, FujZhaWinMur09, CheSchGoeWin07, SchWin09}
%and algorithmic fault-tolerance mechanisms
%\cite{ChenGL08, WinBek03, ChenGoel04, ReiSahYin04, Winfree06, SoloveichikCW08, SchWin09, Luhrs08}, reliable nanoscale engineering through self-organization with DNA tiles shows promise in the near future.

There are different interpretations of ``nondeterminism'' in the aTAM.
We say a tile system is \emph{directed (a.k.a. deterministic)} if it is guaranteed to form one unique final \underline{assembly}, where an assembly is defined not only by which positions are eventually occupied by a tile, but also by which tile type is placed at each position.
We say a tile system \emph{strictly (a.k.a. uniquely) self-assembles} a \underline{shape} if all of its final assemblies are guaranteed to have that shape.
%, although some of the assemblies may place different tile types at the same position, so the tile system may not be directed despite enforcing another sort of determinism by guaranteeing what shape is to assemble.
%
A natural analogy may be made between a non-directed tile system that strictly self-assembles some shape and a nondeterministic Turing machine $N$ that always produces the same output on a given input, regardless of the nondeterministic choices made during computation.
There is always a deterministic Turing machine $M$ computing the same function as $N$ and using no more ``resources'', according to any common resource bound such as time complexity, space complexity, or program length.
Therefore we regard such a restricted class of nondeterministic Turing machines as no more ``powerful'' than deterministic Turing machines.

Based on this analogy, it might seem that strict self-assembly, while allowing one form of nondeterminism (which tile goes where), so strongly requires another form of determinism (which positions have a tile) that extra power cannot be gained by allowing the tile systems to be non-directed.
More precisely, it is natural to conjecture that every infinite shape that is strictly self-assembled by some tile system is also strictly self-assembled by some directed tile system.
In the finitary case, \emph{every} finite shape is assembled by a directed tile system (possibly using as many tile types as there are points in the shape), so to make the idea non-trivial we might conjecture that the tile complexity of a finite shape is independent of whether we consider all tile systems or only those that are directed.
Such conjectures are appealing because the algorithmic design and verification of tile systems \cite{SolWin07} as well as lower bounds and impossibility proofs \cite{jLSAT1,ManStaSto10,AGKS05} %,ManStaSto09poster},
often rely on reasoning about directed tile systems, which are ``better behaved'' in many senses than arbitrary tile systems, even those that strictly self-assemble a shape.
It would be helpful to begin such arguments with the phrase, ``Assume without loss of generality that the tile system is directed.''

However, these conjectures are false.
We show that there is an infinite shape $S$ that is strictly self-assembled by a tile system but not by any directed tile system.
Therefore, in a ``molecular computability theoretic'' sense, nondeterminism allows certain shapes to be algorithmically self-assembled that are totally ``unassemblable'' (to borrow Adleman's tongue-twisting analog of ``uncomputable'' \cite{Adle99}) under the constraint of determinism.
We then show an analogous phenomenon in the finitary case: there is a finite shape $S$ that is strictly self-assembled by a tile system with $c$ tile types, but every directed tile system that strictly self-assembles $S$ has more than $c$ tile types.
In fact to strictly self-assemble the shape in a directed tile system requires more than $\approx \frac{3}{2} c$ tile types.
It is open to improve the constant $\frac{3}{2}$ to be larger or to prove a super-linear gap between the complexity measures; the issue is discussed in more detail in Section \ref{sec-conclusion}.
This establishes a ``molecular complexity theoretic'' analog of the first result.
We then derive a stronger result, showing that the problem of finding the minimum number of tile types that strictly self-assemble a given finite shape is complete for the complexity class $\spt=\NP^\NP$.
In contrast, the problem of finding the minimum number of \emph{directed} tile types that strictly self-assemble a shape was shown to be $\NP$-complete by Adleman, Cheng, Goel, Huang, Kempe, Moisset de Espan\'{e}s, and Rothemund \cite{ACGHKMR02}.

Based on these results, we conclude  that nondeterminism confers extra power to assemble a shape from a small tile system, but unless the polynomial hierarchy collapses, it is computationally more difficult\footnote{``More difficult'' in the sense of nondeterministic time complexity, although it is conceivable that both problems have the same deterministic time complexity.} to exploit this power by finding the size of the smallest tile system, compared to finding the size of the smallest directed tile system.

One might argue that this difference between nondeterministic (but ``output-deterministic'') Turing machines and non-directed (but strict) tile systems is not surprising, since there is a ``monotone'' aspect to tile assembly in the sense that space used to place a tile cannot be reused, whereas a tape cell used to store information by a Turing machine can be reused to store different information later.
It is sometimes said that the difference between space and time
%(in either the narrow sense of computational complexity theory, or in the broad sense of physics and philosophy)
is that ``you can reuse space but you cannot reuse time.''
However, the ``computation'' carried out by tile systems does not distinguish well between space and time.
For instance, the standard simulation of a Turing machine by a tile system (see \cite{RotWin00}) assembles a structure encoding the entire space-time configuration history of the Turing machine.
Even with negative glue strengths that are able to force detachments to occur, the volume requirements of such a simulation must be proportional to $t \cdot s$ for a Turing machine using time $t$ and space $s$ \cite{NIISA}, essentially forcing the solution to contain multiple assemblies that collectively encode the entire computation history.
Tile systems therefore cannot reuse space (tiles), which is the fundamental effect of their monotonicity on their computational abilities.
From this perspective, a Turing machine cannot reuse time any better than any other computational system (barring the use of closed timelike curves \cite{aaronson2009closed}), yet in contrast to tile systems, a nondeterministic but ``output-deterministic'' Turing machine remains no more powerful, even in the sense of time complexity, than a deterministic Turing machine.














==> tam.tex <==
\section{Abstract Tile Assembly Model}
\label{sec-tam-informal}

\newcommand{\fullgridgraph}{G^\mathrm{f}}
\newcommand{\bindinggraph}{G^\mathrm{b}}

This section gives a terse definition of the abstract Tile Assembly Model (aTAM,~\cite{Winf98}). This is not a tutorial; for readers unfamiliar with the aTAM,  \cite{RotWin00} gives an excellent introduction to the model.% and \cite{jSSADST} for a more detailed formalism of the model.


%For a function $f:X \to Y$, for $X' \subseteq X$, $f(X') = \setl{y \in Y}{(\exists x \in X') f(x)=y}$, and for $Y' \subseteq Y$, $f^{-1}(Y') = \setl{x \in X}{f(x) \in Y'}$.
Fix an alphabet $\Sigma$. $\Sigma^*$ is the set of finite strings over $\Sigma$. Given a discrete object $O$, $\langle O \rangle$ denotes a standard encoding of $O$ as an element of $\Sigma^*$. $\Z$, $\Z^+$, and $\N$ denote the set of integers, positive integers, and nonnegative integers, respectively. For a set $A$, $\calP(A)$ denotes the power set of $A$. Given $A \subseteq \Z^2$, the \emph{full grid graph} of $A$ is the undirected graph $\fullgridgraph_A=(V,E)$, where $V=A$, and for all $u,v\in V$, $\{u,v\} \in E \iff \| u-v\|_2 = 1$; i.e., iff $u$ and $v$ are adjacent on the integer Cartesian plane. A \emph{shape} is a set $S \subseteq \Z^2$ such that $\fullgridgraph_S$ is connected. A shape $\Upsilon$ is a \emph{tree} if $\fullgridgraph_\Upsilon$ is acyclic.



A \emph{tile type} is a tuple $t \in (\Sigma^* \times \N)^4$; i.e., a unit square with four sides listed in some standardized order, each side having a \emph{glue} $g \in \Sigma^* \times \N$ consisting of a finite string \emph{label} and nonnegative integer \emph{strength}.
We assume a finite set $T$ of tile types, but an infinite number of copies of each tile type, each copy referred to as a \emph{tile}. An \emph{assembly}
is a nonempty connected arrangement of tiles on the integer lattice $\Z^2$, i.e., a partial function $\alpha:\Z^2 \dashrightarrow T$ such that $\fullgridgraph_{\dom \alpha}$ is connected and $\dom \alpha \neq \emptyset$. The \emph{shape} $S_\alpha \subseteq \Z^2$ of $\alpha$ is $\dom \alpha$.
Two adjacent tiles in an assembly \emph{interact} if the glues on their abutting sides are equal (in both label and strength) and have positive strength.
Each assembly $\alpha$ induces a \emph{binding graph} $\bindinggraph_\alpha$, a grid graph whose vertices are positions occupied by tiles, with an edge between two vertices if the tiles at those vertices interact.\footnote{For $\fullgridgraph_{S_\alpha}=(V_{S_\alpha},E_{S_\alpha})$ and $\bindinggraph_\alpha=(V_\alpha,E_\alpha)$, $\bindinggraph_\alpha$ is a spanning subgraph of $\fullgridgraph_{S_\alpha}$: $V_\alpha = V_{S_\alpha}$ and $E_\alpha \subseteq E_{S_\alpha}$.}
Given $\tau\in\Z^+$, $\alpha$ is \emph{$\tau$-stable} if every cut of $\bindinggraph_\alpha$ has weight at least $\tau$, where the weight of an edge is the strength of the glue it represents.
That is, $\alpha$ is $\tau$-stable if at least energy $\tau$ is required to separate $\alpha$ into two parts. When $\tau$ is clear from context, we say $\alpha$ is \emph{stable}.
Given two assemblies $\alpha,\beta:\Z^2 \dashrightarrow T$, we say $\alpha$ is a \emph{subassembly} of $\beta$, and we write $\alpha \sqsubseteq \beta$, if $S_\alpha \subseteq S_\beta$ and, for all points $p \in S_\alpha$, $\alpha(p) = \beta(p)$.

A \emph{tile assembly system} (TAS) is a triple $\calT = (T,\sigma,\tau)$, where $T$ is a finite set of tile types, $\sigma:\Z^2 \dashrightarrow T$ is the finite, $\tau$-stable \emph{seed assembly}, and $\tau\in\Z^+$ is the \emph{temperature}.
Given two $\tau$-stable assemblies $\alpha,\beta:\Z^2 \dashrightarrow T$, we write $\alpha \to_1^{\calT} \beta$ if $\alpha \sqsubseteq \beta$ and $|S_\beta \setminus S_\alpha| = 1$. In this case we say $\alpha$ \emph{$\calT$-produces $\beta$ in one step}.\footnote{Intuitively $\alpha \to_1^\calT \beta$ means that $\alpha$ can grow into $\beta$ by the addition of a single tile; the fact that we require both $\alpha$ and $\beta$ to be $\tau$-stable implies in particular that the new tile is able to bind to $\alpha$ with strength at least $\tau$. It is easy to check that had we instead required only $\alpha$ to be $\tau$-stable, and required that the cut of $\beta$ separating $\alpha$ from the new tile has strength at least $\tau$, then this implies that $\beta$ is also $\tau$-stable.}
If $\alpha \to_1^{\calT} \beta$, $ S_\beta \setminus S_\alpha=\{p\}$, and $t=\beta(p)$, we write $\beta = \alpha + (p \mapsto t)$.
The \emph{$\calT$-frontier} of $\alpha$ is the set $\partial^\calT \alpha = \bigcup_{\alpha \to_1^\calT \beta} S_\beta \setminus S_\alpha$, the set of empty locations at which a tile could stably attach to $\alpha$.
%The \emph{$t$-frontier} $\partial_t \alpha \subseteq \partial \alpha$ of $\alpha$ is the set $\setr{p\in\partial \alpha}{\alpha \to_1^\calT \beta \text{ and } \beta(p)=t}.$

A sequence of $k\in\Z^+ \cup \{\infty\}$ assemblies $\alpha_0,\alpha_1,\ldots$ is a \emph{$\calT$-assembly sequence} if, for all $1 \leq i < k$, $\alpha_{i-1} \to_1^\calT \alpha_{i}$.
We write $\alpha \to^\calT \beta$, and we say $\alpha$ \emph{$\calT$-produces} $\beta$ (in 0 or more steps) if there is a $\calT$-assembly sequence $\alpha_0,\alpha_1,\ldots$ of length $k = |S_\beta \setminus S_\alpha| + 1$ such that
1) $\alpha = \alpha_0$,
2) $S_\beta = \bigcup_{0 \leq i < k} S_{\alpha_i}$, and
3) for all $0 \leq i < k$, $\alpha_{i} \sqsubseteq \beta$.
If $k$ is finite then it is routine to verify that $\beta = \alpha_{k-1}$.\footnote{If we had defined the relation $\to^\calT$ based on only finite assembly sequences, then $\to^\calT$ would be simply the reflexive, transitive closure $(\to_1^\calT)^*$ of $\to_1^\calT$. But this would mean that no infinite assembly could be produced from a finite assembly, even though there is a well-defined, unique ``limit assembly'' of every infinite assembly sequence.} We say $\alpha$ is \emph{$\calT$-producible} if $\sigma \to^\calT \alpha$, and we write $\prodasm{\calT}$ to denote the set of $\calT$-producible assemblies. The relation $\to^\calT$ is a partial order on $\prodasm{\calT}$ \cite{Roth01,jSSADST}.
%Note that all $\calT$-producible assemblies are $\tau$-stable.
A $\calT$-assembly sequence $\alpha_0,\alpha_1,\ldots$ is \emph{fair} if, for all $i$ and all $p\in\partial^\calT\alpha_i$, there exists $j$ such that $\alpha_j(p)$ is defined; i.e., no frontier location is ``starved''.

%Given a TAS $\calT=(T,\sigma,\tau)$, an assembly $\alpha$ is \emph{$\calT$-producible}, or \emph{producible} if $\calT$ is clear from context, if either $\alpha = \sigma$, or $\alpha$ results from the $\tau$-stable attachment of a single tile to a producible assembly (``$\tau$-stable attachment'' meaning that the cut separating the tile from the rest of the assembly has strength $\geq \tau$, which implies by induction that $\alpha$ is $\tau$-stable).
An assembly $\alpha$ is \emph{$\calT$-terminal} if $\alpha$ is $\tau$-stable and $\partial^\calT \alpha=\emptyset$.
We write $\termasm{\calT} \subseteq \prodasm{\calT}$ to denote the set of $\calT$-producible, $\calT$-terminal assemblies.
A TAS $\calT$ is \emph{directed (a.k.a., deterministic, confluent)} if the poset $(\prodasm{\calT}, \to^\calT)$ is directed; i.e., if for each $\alpha,\beta \in \prodasm{\calT}$, there exists $\gamma\in\prodasm{\calT}$ such that $\alpha \to^\calT \gamma$ and $\beta \to^\calT \gamma$.\footnote{The following two convenient characterizations of ``directed'' are routine to verify.
%It is routine to verify that the following two convenient definitions of ``directed'' are equivalent to the stated definition.
$\calT$ is directed if and only if $|\termasm{\calT}| = 1$. $\calT$ is \emph{not} directed if and only if there exist $\alpha,\beta\in\prodasm{\calT}$ and $p \in S_\alpha \cap S_\beta$ such that $\alpha(p) \neq \beta(p)$.} %; i.e., if there are two producible
%(not necessarily terminal)
%assemblies with different tile types in the same position.}
We say that a TAS $\calT$ \emph{strictly (a.k.a. uniquely) self-assembles} a shape $S \subseteq \Z^2$ if, for all $\alpha \in \termasm{\calT}$, $S_\alpha = S$; i.e., if every terminal assembly produced by $\calT$ has shape $S$.
If $\calT$ strictly self-assembles some shape $S$, we say that $\calT$ is \emph{strict}.
Note that the implication ``$\calT$ is directed $\implies$ $\calT$ is strict'' holds, but the converse does not hold.

In this paper we will always use \emph{singly-seeded temperature-2} TAS's, those with $|S_\sigma|=1$ and $\tau=2$; hence we will use the term \emph{seed tile} for $\sigma$ as well, and for the remainder of this paper we use the term TAS to mean singly-seeded temperature-2 TAS.
When $\calT$ is clear from context, we may omit $\calT$ from the notation above and instead write
$\to_1$,
$\to$,
$\partial \alpha$,
\emph{frontier},
\emph{assembly sequence},
\emph{produces},
\emph{producible}, and
\emph{terminal}.
Since the behavior of a TAS $\calT=(T,\sigma,2)$ is unchanged if every glue with strength greater than 2 is changed to have strength exactly 2, we assume henceforth that all glue strengths are 0, 1, or 2, and use the terms \emph{null glue}, \emph{single glue}, and \emph{double glue}, respectively, to refer to these three cases.\footnote{We use \emph{null bond}, \emph{single bond}, and \emph{double bond} similarly to refer to the \emph{interaction} of two tiles.}
We also assume without loss of generality that every single glue or double glue occurring in some tile type in some direction also occurs in some tile type in the opposite direction, i.e., there are no ``effectively null'' single or double glues.\footnote{Thus the existence of a tile with a double glue facing empty space implies that the empty space is part of the frontier. Many of our arguments use the contrapositive that if a shape $S$ is strictly self-assembled by a tile system and a side of a tile faces a point $p \not\in S$, then the tile cannot have a double glue on that side.}









